OOD-HOI: Text-Driven 3D Whole-Body Human-Object Interactions Generation Beyond Training Domains

Generating realistic 3D human-object interactions (HOIs) from text descriptions is a active research topic with potential applications in virtual and augmented reality, robotics, and animation. However, creating high-quality 3D HOIs remains challenging due to the lack of large-scale interaction data and the difficulty of ensuring physical plausibility, especially in out-of-domain (OOD) scenarios. Current methods tend to focus either on the body or the hands, which limits their ability to produce cohesive and realistic interactions. In this paper, we propose OOD-HOI, a text-driven framework for generating whole-body human-object interactions that generalize well to new objects and actions. Our approach integrates a dual-branch reciprocal diffusion model to synthesize initial interaction poses, a contact-guided interaction refiner to improve physical accuracy based on predicted contact areas, and a dynamic adaptation mechanism which includes semantic adjustment and geometry deformation to improve robustness. Experimental results demonstrate that our OOD-HOI could generate more realistic and physically plausible 3D interaction pose in OOD scenarios compared to existing methods.

==> sec/1_intro.tex <==
\section{Introduction}

% 1. The background of HoI, including industry and academic
% 2. The mainstream of HOI and its challenging, lead to text driven HOI;
%3. Three core challenges for HOI (w/ wo text):
    % 1) Dataset;
    % 2) one-to-N or N-to-One;
    % 3) Generalization (or physical constraint)
% 4. In this paper, we proposed a \mymethod{} method to tackle xxx problem (achieve xxxx). It includes one, two, three modules. Specifically, xxxx
% 5. The contributions. 


When we play overcooks, the pre-made animation shows the little characters in the kitchens are holds a frying pan with right hand and sprinkles salt on it with the left hand are cutey and adding some fun to the chaos. During the daily life interaction, the hand pose is often defined as a function of object's pose, shape and category. Not only do they need to look realistic, but also interact realistically. While existing works~\cite{guo2022generating, petrovich2022temos, tevet2023human} have been successful in modeling diverse and realistic 3D human body motions from text prompt without considering the hand motions. Often, these bodies are considered in ``isolation`` without object context, which significantly limits the expressiveness in the semantics of generated motion sequence. Other works generating only hand grasps often ignores the body~\cite{christen2024diffh2o,cha2024text2hoi}, but in fact, the consistency of hands and the whole body is very important. We argue that these are all just parts of the problem. What we really need, instead, is to generate contact of full-body avatars grasping objects, by jointly considering the body, hands and the object from the text prompt.

Learning to generate the 3D hand-object interaction from a text prompt is extremely challenging due to the scarcity of the dataset: the diversity of existing datasets for the contact of 3D meshes and associated text labels is far behind the one of real-world distribution which is determined by a number of parameters such as hand type (e.g., left or right), object’s category and structure, contact regions, and so on. A generative model learned from such limited data will fail in the diverse modeling of physically and semantically plausible 3D hand-object interaction. In order to deal with dynamically changing environment for planning~\cite{wan2023unidexgrasp++, lu2023ugg}, we aims to produce diverse grasping postures with same text labels.

To overcome this challenge, we propose to decompose the interaction generation task into three sub tasks, "coarse 3D HOIs generation", “contact prediction diffusion model” and “contact-guided refined model”, and the models dedicated to each task learn a general geometry representation from the augmented dataset, which leads to the significant improvement in the generalizability and physical plausibility of the combined pipeline.

For the coarse 3D HOIs generation, we newly develop a dual-branch transformer based diffusion model(HOIs-DM) to generate a coarse huamn and object pose conditioning on the input text prompt and object shape. To encourage coherent pose of contact, we develop a cross-attention communication module, exchanging information between the human and object pose generation models. Unlike a conventional diffusion process~\cite{ho2020denoising}, the model is designed to directly estimate the final sample at each step, which allows us to apply explicit geometric loss (e.g., relative distance or orientation) to improve the geometric correctness. Our diffusion model learns the augmented data where we deform the shape of the object in the original dataset without changing the contact information.

For the Contact Prediction Diffusion Model (CPDM), we propose a contact map prediction network that encodes the local geometric surface of a 3D object mesh, along with a target motion description and a corresponding hand pose. This network generates joint locations and probabilities, indicating potential contact areas on the object surface. To address the issue of hand shape variations causing unintended penetration during contact, we use joint locations to define the contact areas between the human hand and the object, effectively mitigating this problem. By conditioning on hand poses, our contact prediction module naturally decodes reasonable contact areas.

In the contact-guided refinement model, we incorporate the estimated contact information and employ classifier guidance to achieve precise and stable contact between the human hand and objects, significantly reducing issues like floating hands and object penetration. Instead of designing a monolithic model, our proposed approach disentangles the generation of human and object poses from the estimation of their contact points, leading to improved accuracy and interaction quality.

Using these three modules, we introduce a text-guided human-object interaction generation framework that generates 3D interactions in a compositional manner. Given a text prompt and a canonical 3D object mesh, our HOIs-DM model generates an initial coarse contact pose. Our contact prediction diffusion model encodes the hand pose, text, and object mesh with agent-wise (object, left hand, right hand) positional embeddings to generate contact positions and probabilities for each human joint. Finally, our refinement model enhances the physical accuracy of the 3D interaction using classifier guidance, refining the contacts and suppressing penetration artifacts.

In the experiments, we validate our model on two datasets(H2O~\cite{Kwon_2021_ICCV}, GRAB~\cite{taheri2020grab}), we choose the pose that only grasp the object stable which means the object is away from the origin height and have two fingers grasp at least. Our methods outperforms other baseline methods in terms of accuracy, diversity, and physical realism by large margins. We also demonstrate that our compositional framework enables the application of our method to new text that are not seen during training.

Our contribution can be summarized as follows:
\begin{enumerate}
    \item We proposed three stage coarse to fine method for investigating human-object interaction tasks through a perspective of generation from a text prompt.
    \item We propose a new contact anchors representation instead of using the conventional contact map as navigational cues for affordance information.
    \item We annotate the textual descriptions for each stable HOI pose from existing human and object motion datasets, which will be made public.
\end{enumerate}

==> sec/3_methods.tex <==
\section{Method}

\begin{figure*}[htbp]
\centering
\includegraphics[width=\textwidth]{figs/method.pdf}
\caption{Overview of HOI-Diff for 3D Human-Object Interaction (HOI) generation using diffusion models. Our approach decomposes the generation process into three stages: (a) a dual-branch model that exchanges information through a Reciprocal Module to generate an initial interaction pose; (b) representation of physically grounded contact points based on text input, object geometry, and the initial hand pose; and refinement of the human-object interaction, integrating estimated contact information and leveraging classifier guidance to achieve accurate, close contact between humans and objects, resulting in coherent HOIs.}
\label{fig:method}
\end{figure*}

\subsection{Overview}
\textbf{Pose Representations.} We denote a 3D HOI pose as $x = \left\{x^h, x^o\right\}$. It consists of human $x^h \in \mathbb{R}^{159}$ and object pose $x^o \in \mathbb{R}^{6}$. For $x^h$, we adopt the SMPL-H~\cite{MANO:SIGGRAPHASIA:2017} pose components which include human global orient, body pose, hand pose and corresponding human transl. For the object pose $x^o$, we assume the object geometry is given as an input, and thus we only need to estimate its 6 DoF poses in the generation. We represent each object instance as a point cloud of 4000 points \cite{cha2024text2hoi} $p_o \in \mathbb{R}^{4000 \times 3}$.

%三部分a,b,c明确表示
\textbf{Overview of 3D HOI Pose Generation.} Our method, illustrated in Fig.~\ref{fig:method}, follows a three-stage, contact-guided approach for coarse-to-fine generation. First, we employ a dual-branch model that integrates human and object features through a Reciprocal Module (RM) to generate initial human-object interactions (Sec.~\ref{sec:coarse generation}). In the second stage, we introduce a novel contact prediction model that identifies potential contact points across 30 hand joints, ensuring realistic physical contact (Sec.~\ref{sec:contact prediction}). Finally, the contact positions generated in the second stage serve as classifier guidance to refine human-object interactions during each step of human and object pose generation (Sec.~\ref{sec:interaction refiner}).


% \textbf{Overview of 3D HOI pose Generation.} As shown in Fig~\ref{fig:method}, Our method consists of three modules as from contact guided coarse to fine generation. In Sec.~\ref{sec: coarse generation}, we introduce a dual-branch Human-object Interaction Diffusion Model (HOIs-DM), which couples the human pose and object pose, could produce diverse yet stable interaction poses, capturing the intricate interplay and mutual grasp interactions between humans and objects. To ensure diverse physical plausible contact between humans and objects, we propose a novel contact prediction diffusion model (CPDM) in Sec.~\ref{sec: contact prediction}, whose output will be used as classifier guidance (Sec.~\ref{sec: interaction refiner}) to refine the interactions at each step of human/object pose generation.

\begin{figure}[H]
\includegraphics[width=0.5\textwidth, trim=200 20 100 0, clip]{figs/HOIs-DM.pdf}
\caption{Illustration of dual-branch HOIs model architecture for first stage generation. It has two branches designed for generating human and object pose individually. A bidirectional attention is introduced to allow information exchange between two branches to generate coherent result.}
\label{fig:coarse-generation}
\end{figure}

% \subsection{Coarse 3D HOIs Generation}
\subsection{Dual-branch HOIs Model}
%考虑主要贡献
\label{sec:coarse generation}
% 介绍对偶结构和区别（为什么要用对偶结构）module内容介绍
Due to the differing distributions between human and object poses~\cite{taheri2020grab}—for example, grasping an apple may require a similar hand pose regardless of the apple's position—we propose a dual-branch model to generate coherent human and object poses. This model decomposes the overall pose generation into two distinct Transformer modules~\cite{vaswani2017attention}: a human pose generation module and an object pose generation module, which makes the generation process more focused on its rationality of the posture. At each diffusion step $t$, the model receives a conditional input $c$ and noisy poses $x$ as input. The diffusion model $p_{\theta}(x_{t-1}|x_{t}, c)$ learns the reverse diffusion process, progressively generating clean data from Gaussian noise $x_t$ through $T$ sequential denoising steps.

\begin{equation}
\label{eq1}
 p_{\theta}(x_{t-1}|x_{t}, c) = \mathcal{N}\left(x_{t-1}; \mu_{\theta}(x_{\theta}(x_{t}, t, c)), (1-\alpha_{t})I\right)
\end{equation}

In the human pose generation module, the condition $c$ comprises only the text description $d$. For the object pose generation module, $c$ includes both the text description $d$ and the object’s point clouds $p_o$. Here, $t$ denotes the current denoising step, and $x_t$ includes both human pose $x^h$ and object pose $x^o$ components.

% First, we introduce a dual-branch Human-Object Interaction Diffusion Model (HOIs-DM) for generating approximately coherent human and object motions. As shown in Fig.~\ref{fig:coarse-generation}, HOIs-DM comprises two Transformer models \cite{vaswani2017attention}: a human pose generation module, $M^h$, and an object pose generation module, $M^o$. At each diffusion step $t$, these modules take as input the text description $d$, the object point cloud $p$, and noisy poses $x^h$ and $x^o$, predicting clean human and object poses $x^h_0$ and $x^o_0$, respectively. The diffusion model $p_{\theta}(x_{t-1}|x_{t}, c)$ learns the reverse diffusion process to generate clean data from a Gaussian noise $x_t$ with $T$ consecutive denoising steps

% RM结构设计理由， 公式说明f和f^、hat{o}关系, f介绍怎么来
To address the challenge of declining interaction information when decoupling human and object pose generation, we introduce a Reciprocal Module (RM) to facilitate feature exchange between the human and object pose generation modules. The RM functions as a Transformer block, receiving intermediate features $f = \{f^h, f^o\}$ from both modules and refining these through a cross-attention mechanism to retain human-object interaction information. Specifically, the RM refines the input features, generating updated representations $\hat{f} = \{\hat{f}^h, \hat{f}^o\}$, which are conditioned on each other. These updated features are subsequently passed to the next layers of their respective branches to produce the final, clean poses $x = \{x^h, x^o\}$.

\begin{align}
\hat{f}^h = \text{Cross-Attention}(Q_{f^h}, K_{f^h}, V_{f^o}) 
\\
\hat{f}^o = \text{Cross-Attention}(Q_{f^o}, K_{f^o}, V_{f^h})
\end{align}

The integration of the RM enables a more precise human-object interaction in the generated poses; this design choice is evaluated in Tab.~\ref{tab:Ablation}. Additionally, to handle the different dimensionalities of human and object poses, we adapt the input and output linear layers accordingly. Further methodological details of the dual-branch model are provided in the supplementary material.

% To enhance human-object interaction during motion generation, we introduce a Reciprocal Module (RM) designed to enable feature exchange between $M^h$ and $M^o$. The RM operates as a Transformer block that receives intermediate features, $f^h$ and $f^o$, from $M^h$ and $M^o$ and processes these inputs using a cross-attention mechanism to generate refined representations. The updated feature representations, $f^{\hat{h}}$ and $f^{\hat{o}}$, for the human and object are subsequently conditioned on each other and passed to the next layers of their respective branches to estimate the final clean poses $x^h_0$ and $x^o_0$.

% With the integration of RM, the generated human and object poses are more precisely coupled; we evaluate this design choice in Sec.~\ref{tab:Ablation}. To account for the differing dimensions of human and object poses, we adjust the input and output linear layers to handle these variations. Further methodological details of HOIs-DM are provided in the supplementary material.

% \subsection{Contact Prediction Diffusion Model}
\subsection{Physical-enhanced Contact Prediction}
%物理引导靠
\label{sec:contact prediction}

%明确说之前生成结果， 加上图说明，用抓取图去说明约束
We make two key empirical observations: (1) Generated models often struggle to predict accurate SMPL-H parameters, likely due to the non-Euclidean nature of this parameter space. (2) In contrast, generated models predict interaction features in Euclidean space with significantly higher accuracy, aligning with recent findings~\cite{zhang2021we, taheri2021goal}. Due to these observations, initial generation results often lack physical plausibility, leading to issues such as floating objects or interpenetration. To address these challenges in complex interactions, accurately identifying contact areas between the human and object is crucial. Text2HOI~\cite{cha2024text2hoi} defines contact regions based on distance measurements between human and object surfaces; however, this approach heavily depends on the quality of generated poses and cannot correct errors from the initial pose. Inspired by HOI-Diff~\cite{peng2023hoi}, which estimates contact areas by calculating the minimum distances between body joints and object points, we define contact regions based on the closest points between hand joints and object points.

This approach offers essential physical insights, as it identifies specific regions where human-object interaction is likely to occur, enhancing the realism and stability of the generated poses. Unlike general body contacts, stable and dexterous hand poses for grasping require the thumb and at least one additional finger to establish a secure grip. Moreover, contact areas vary even with identical objects and interaction types; for example, a "pick" action can occur from the top or side of an object, each requiring distinct hand poses depending on the intended action.

Estimating contact in 3D point clouds is inherently challenging~\cite{deng20213d, tripathi2023deco, jiang2023full}, particularly in the context of 3D HOI generation involving textual prompts. In this work, we consider three joints per finger across both hands—thumb, index, middle, ring, and pinky—resulting in a total of 30 joints that act as the interacting elements in HOI scenarios. This setup effectively models common interactions such as grasping with both hands or lifting with a single hand. We use binary contact labels to indicate which joints are in contact with the object and predict 30 corresponding points on the object’s surface, identified as the closest points to the selected hand joints. The binary contact labels for different hand joints are interdependent, with the thumb always included in grasping, enabling effective handling of complex HOIs.

Specifically, at each diffusion step $n$ in contact prediction, the noisy data consists of human contact labels, representing the contact status of the 30 primary hand joints and denoted as $y \in \left\{ 0,1 \right\}^{30}$, as well as the 30 corresponding contact points on the object surface, denoted as $y^o_n \in \mathbb{R}^{30 \times 3}$. The model is designed to predict both contact probabilities and contact positions. Contacting hand joints are dynamically selected by applying a threshold $\tau$ (set to 0.8) to the predicted probabilities, and the corresponding contact points on the object are determined based on these selected joints. This contact prediction model operates analogously to the diffusion denoising process described in Eq.~\ref{eq1}.


% Due to the complexity of human-object interactions, HOIs-DM alone often fails to produce physically plausible results, leading to issues such as floating objects or penetrations. To enhance the generation of intricate interactions, it is crucial to identify contact areas between the human and object. TEXT2HOI~\cite{cha2024text2hoi} defines contact areas based on distance measurements between the surfaces of the human and object. However, this approach heavily relies on the quality of the generated human and object poses and cannot correct errors in the coarse 3D HOI results. Inspired by HOI-Diff~\cite{peng2023hoi}, which estimates body contact areas from the closest distances between predicted body joints and object points, we define the contact area based on the closest points between hand joints and object points. Unlike body contacts, stable and dexterous hand poses require the use of the thumb and at least one other finger for grasping. Furthermore, contact areas vary even with the same object and interaction type; for instance, a "pick" action can occur from the top or side of an object, with different hand poses based on the intent. 

% To address this, we introduce a Contact Prediction Diffusion Model (CPDM) for contact prediction. Given a text description $d$, an object point cloud $p$, and a coarse hand pose $h$, CPDM generates the corresponding contact area for the hand pose, thus compensating for potential errors in HOIs-DM. Additionally, it stochastically generates contact points to ensure diversity in the generated poses.

% Estimating contact in 3D point clouds is inherently challenging~\cite{deng20213d, tripathi2023deco, jiang2023full}, especially in the context of 3D HOI generation involving textual prompts. In this work, we consider three joints per finger across both hands—thumb, index, middle, ring, and pinky—for a total of 30 joints, which act as the interacting elements in HOI scenarios. This setup effectively models common interactions such as grasping with both hands or lifting with a single hand. We use binary contact labels to indicate which joints are in contact with the object and predict 30 corresponding points on the object’s surface, identified as the closest points to the selected hand joints. The binary contact labels for different hand joints are interdependent, with the thumb always included in grasping, allowing us to handle complex HOIs.

% Specifically, at each diffusion step $n$ of contact prediction, the noisy data consists of human contact labels representing the contact status for the 30 primary hand joints, denoted as $y \in \left\{ 0,1 \right\}^{30}$, and the 30 corresponding contact points on the object surface, denoted as $y^o_n \in \mathbb{R}^{30 \times 3}$. The model is designed to predict both contact probabilities and contact positions. Contacting hand joints are dynamically selected by applying a threshold $\tau$ (set to 0.8) to the predicted probabilities. The corresponding contact points on the object are then determined based on the selected joints. This contact prediction model operates similarly to the diffusion denoising process described in Eq.~\ref{eq1}.

\subsection{Contact-guided Interaction Refiner}

%之前得到模型存在什么问题，为了解决这些问题提出什么方法来解决， refiner过程只需要介绍loss和对应参数
\label{sec:interaction refiner}
% verctor guided penetration correction
To achieve accurate and close contact between humans and objects—thus reducing issues of floating objects and penetrations—we propose the classifier guidance generation~\cite{diller2024cg}.

In brief, we define an analytic function $G(\mu^h_t, \mu^o_t, y_0)$ that evaluates the alignment between generated hand joints and the object’s 6 DoF pose. This function enforces close proximity in contact positions between the human and object while preventing penetrations. Based on the gradient of $G(\mu^h_t, \mu^o_t, y_0)$, we adjust the generated human and object poses at each diffusion step $t$, following the method in~\cite{karunratanakul2023guided}.

% \begin{equation}
% \label{eq2}
% \mu_t = \mu_t - \tau {\textstyle \sum_t} \nabla_{\mu_t} G(\mu^h_t, \mu^o_t, y_0)
% \end{equation}

% Here, $\tau$ controls the guidance strength for both human and object poses. During the denoising stage, to counteract any bias of the diffusion model that might suppress the guidance signal, we iteratively perturb $K$ times in the final denoising step. Instead of predicting the noise $\epsilon_t$ at each diffusion step, our diffusion model $M_{\theta}$, with parameters $\theta$, predicts the final clean pose $x_0 = M_{\theta}(x_t, t, c)$. We sample $x_{t-1} \sim N(\mu_t, {\textstyle \sum_t})$ and compute the mean as

% \begin{equation}
% \label{eq3}
% \mu_t = \frac{\sqrt{\alpha _{t-1}}\beta_t }{1 - \alpha _t} x_0 + \frac{\sqrt{1-\beta _t}(1-\alpha _{t-1}) }{1-\alpha_t}x_t  
% \end{equation}

% where $\alpha =  {\textstyle \prod_{s=1}^{t}}(1-\beta_s)$ and $\beta \in (0,1)$ represents the variance schedule. ${\textstyle \sum_t} = \frac{1-\alpha_{t-1}}{1-\alpha_t}\beta_t$ denotes the chosen variance schedule.

We consider three terms for the objective function $G(\mu^h_t, \mu^o_t, y_0)$. First, to ensure proximity between human and object contact points in the generated 3D HOIs, we minimize the distance between human contact vertices and object contact points. Given that we predict hand joints in a later stage, we use fixed mapping points for the hand joints, as hand deformation is minimal compared to body shape deformation.

\begin{equation}
\label{eq4}
G_{con} = \sum_{i \in \{1,2,\dots,30\}} \| R(\mu^h_t(i)) - V(y^o_t(i))\| ^2
\end{equation}

where $\mu^h_t(i)$ and $y^o_t(i)$ represent the $i$-th available contacting hand vertex and object contact point, respectively. $R(\cdot)$ transforms human vertices to global coordinates, while $V(\cdot)$ retrieves the object contact point from the predicted mean of the object pose $\mu^o_t$.

To address penetration issues, we introduce a normal plane alignment criterion at contact points. Observing that penetration often occurs due to incorrect contact angles, we enforce the sum of normal planes at contact points to zero, ensuring that contact occurs on the object’s surface. This objective is formulated as

\begin{equation}
\label{eq5}
G_{norm} = \sum_{i \in \{1,2,\dots,30\}} \| N_h R(\mu^h_t(i)) - N_o V(y^o_t(i))\| ^2
\end{equation}

where $N_h$ and $N_o$ denote the normal planes for human vertices and object points, respectively.

Third, we employ the Body Balance Loss~\cite{Zheng_2023_ICCV} to ensure stability in body poses. This requires the gravity line to align with the base of support. The vertical projection of the body’s center of gravity (approximated by the hip joint) must pass through the base of support formed by four predefined support points located at the forefoot and heel. The body balance loss is defined as

\begin{equation}
\label{eq6}
G_{balance}(\theta^b) = D(J^b_{hip-xy}, S)
\end{equation}

where $D(p, P)$ calculates the distance between point $p$ and polygon $P$, yielding zero if $p$ lies within $P$. Here, $J^b_{hip-xy}$ is the vertical projection of the hip onto the ground, and $S$ denotes the base of support defined by ground contact points on the feet.

Finally, we combine all these objectives into the final objective function:

\begin{equation}
\label{eq7}
G = G_{con} + \alpha G_{norm} + \beta G_{balance}
\end{equation}

where $\alpha$ and $\beta$ are weighting factors for balancing the contributions of each term.


% physical refiner
% 1.coarse result problem
% 2.refiner process (约束点+生成函数)
% 3.loss function内容

% data augmentaion
% 扩大in domain 增强效果
